TruePose: Human-Parsing-guided Attention Diffusion for Full-ID Preserving Pose Transfer

Pose-Guided Person Image Synthesis (PGPIS) generates images that maintain a subject's identity from a source image while adopting a specified target pose (e.g., skeleton). While diffusion-based PGPIS methods effectively preserve facial features during pose transformation, they often struggle to accurately maintain clothing details from the source image throughout the diffusion process. This limitation becomes particularly problematic when there is a substantial difference between the source and target poses, significantly impacting PGPIS applications in the fashion industry where clothing style preservation is crucial for copyright protection. Our analysis reveals that this limitation primarily stems from the conditional diffusion model's attention modules failing to adequately capture and preserve clothing patterns. To address this limitation, we propose human-parsing-guided attention diffusion, a novel approach that effectively preserves both facial and clothing appearance while generating high-quality results. We propose a human-parsing-aware Siamese network that consists of three key components: dual identical UNets (TargetNet for diffusion denoising and SourceNet for source image embedding extraction), a human-parsing-guided fusion attention (HPFA), and a CLIP-guided attention alignment (CAA). The HPFA and CAA modules can embed the face and clothes patterns into the target image generation adaptively and effectively. Extensive experiments on both the in-shop clothes retrieval benchmark and the latest in-the-wild human editing dataset demonstrate our method's significant advantages over 13 baseline approaches for preserving both facial and clothes appearance in the source image.

==> sec/0_abstract.tex <==
\begin{abstract}
%
Pose-Guided Person Image Synthesis (PGPIS) aims to generate a target image having the same pose as the given pose condition (\eg, skeleton) and the same person as the given source image.
%
Diffusion-based PGPIS methods can effectively preserve face IDs from source images following the specified pose, but they struggle to maintain high-quality clothing IDs.
%
Specifically, the generated clothing patterns and textures often differ significantly from those in the source images. 
%
We identified a critical challenge: SOTA methods use pre-trained models (\eg, CLIP) for image encoding, which well captures face features but overlooks clothing details.
%
% (2) There is a significant discrepancy between the person's pose in the source and target poses, making synthesis particularly challenging.
%
In this work, we propose a novel PGPIS framework denoted as the person-parsing-guided Siamese network diffusion model that can generate high-quality and ID-preserved faces and clothing.
%
The intuitive idea is to use an UNet having the same architecture in the diffusion model for image encoding and leverage person-parsing maps to guide the diffusion denoising process. 
%
To this end, our method involves three modules: \textit{First}, we design a Siamese network containing two UNet branches (\ie, SourceNet and TargetNet) with the same architectures. 
%
% akes the reference image, parsing-aligned pose embeddings, and parsing-aligned CLIP embeddings as the inputs and
SourceNet outputs multi-layer features considering the embeddings of the source image and parsing maps. These features are fed to each layer of TargetNet for noise prediction in the diffusion model. 
% The learnable SourceNet helps preserve both face ID and clothing ID. 
%
\textit{Second}, we propose the pose-guided parsing projection that can estimate the target image's person-parsing map by transferring the source image's parsing map based on the target and source poses. 
% The generated parsing map is employed to extract the parsing-aligned pose embeddings and CLIP embeddings used in SourceNet.
%
\textit{Third}, we propose the person-parsing-aligned CLIP embedding extraction. 
%
We use the parsing maps of the source and target images to crop the person in the source image and extract its CLIP-text \& -visual embeddings to highlight the face and clothing features for both SourceNet and TargetNet.
%
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Images of well-dressed individuals are widely used in shopping stores for advertising. To achieve a high-quality image, a model must wear specific clothing and adopt a designated pose. Once these images are captured and deployed, it becomes difficult for stores to change the model's pose.
%
Otherwise, they must invite the model to wear the same clothes and undergo the photography process again, which is time-consuming and costly.
%
The well-defined task, \ie, pose-guided person image synthesis (PGPIS), could easily meet the above requirement efficiently. 
%
PGPIS aims to generate an image that matches the specified pose condition (\eg, skeleton) while retaining the same appearance (person and clothing) as the source image (See the inputs in \figref{fig:fig_intro}) \cite{ma2017pose,liu2019liquid,zhu2019progressive}.
%
Such a task is challenging due to the potential significant discrepancy between the source and target poses.

Previous works formulate the task as the deep generation problem and employ generative adversarial network (GAN) \cite{zhou2022cross,zhang2022exploring,zhang2021pise,sarkar2021style,tang2020xinggan,zhu2019progressive,siarohin2018deformable} and variational autoencoder (VAE) \cite{esser2018variational} to achieve the goal. 
%
However, GAN-based methods struggle with unstable training and generating high-quality images. VAE-based methods usually suffer from some artifacts like blur. 

Recently, diffusion models have demonstrated powerful capabilities in generating high-quality images \cite{ho2020denoising,song2020score} with flexible control conditions \cite{rombach2022high}.
%
Researchers have developed diffusion-based PGPIS methods, achieving impressive results \cite{bhunia2023person,lu2024coarse,shen2024advancing}.
%
\begin{figure}{r}{}
    \centering
    % \vspace{-10pt}
    \includegraphics[width=1.0\linewidth]{figures/fig_intro.pdf}
    \caption{Comparison with CFLD  \cite{lu2024coarse} and PCDM (ICLR'24) \cite{shen2024advancing}. They fail to preserve the clothing patterns and textures. The main reason is that the image encoder overlooks the clothing details (See the ``Feature Attention Map (Feat. Att. Map)").  In contrast, our method can generate high-quality images with preserved face and clothing IDs.}
    % \vspace{-10pt}
    \label{fig:fig_intro}
\end{figure}
%
In particular, the state-of-the-art (SOTA) methods, \eg, coarse-to-fine latent diffusion (CFLD) \cite{lu2024coarse} and progressive conditional diffusion (PCDM) \cite{shen2024advancing}, can generate realistic images with preserved human pose and face ID (See in \figref{fig:fig_intro}).
%
However, they struggle to transfer clothing patterns and textures (\ie, clothing ID) from the source image to the target image.
%
% For example, in the $1^\text{st}$ case in \figref{fig:fig1}, the t-shirt in the source image contains a sentence. The generated image by CFLD only captures the style of the t-shirt but loses all of the words, while PCDM can transfer some words but fails to recover the intermediate ones.
%
We display four cases in \figref{fig:fig_intro} and observe that: \ding{182} CFLD and PCDM can hardly preserve clothing patterns and textures. The two methods fail to transfer the texts ($1^\text{st}$ and $4^\text{th}$ cases), regular texture ($2^\text{nd}$ case), and irregular textures ($3^\text{rd}$ case).
%
% PCDM presents relatively better clothing ID-preserving capability than CFLD. 
%
\ding{183} As the discrepancy between the source and target poses increases, it becomes more challenging to preserve the clothing IDs. For example, with similar source images ($1^\text{st}$ case vs. $4^\text{th}$ case), PCDM can reproduce some words in the $1^\text{st}$ case but loses all words in the $4^\text{th}$ case.
%
\ding{184} We calculate the feature attention map of baseline methods for each case, which shows that both methods pay less attention to the clothing regions. We will conduct a statistical analysis in \secref{sec:limitation} for further discussion.


These observations inspire us to design a novel PGPIS framework that preserves both facial and clothing identities. Our approach leverages person-parsing maps of both source and target images to guide the encoding process, ensuring the features focus on both face and clothing regions.
%
We propose a person-parsing-guided Siamese network diffusion model with three main contributions: \textit{First}, we design a Siamese network comprising two UNet branches (\ie, SourceNet and TargetNet) with identical architectures. SourceNet generates multi-layer features by incorporating features from the source image and parsing maps. These features are subsequently fed into each layer of TargetNet for noise prediction in the diffusion model.
%
\textit{Second}, we introduce the pose-guided parsing projection, which estimates the person-parsing map of the target image by transferring the source image’s parsing map based on the poses of both the source and target images.
%
\textit{Third}, we propose person-parsing-aligned CLIP embedding extraction. This technique uses the parsing maps of the source and target images to crop the person in the source image, extracting CLIP-text and visual embeddings to emphasize facial and clothing features for both SourceNet and TargetNet.
%
We validate our method on the in-shop clothes retrieval benchmark with two resolutions ($512\times352$, $256\times176$) and compare with 11 SOTA baselines.
%
As shown in \figref{fig:fig_intro}, our method can generate high-quality images with well-preserved facial appearance and clothing patterns.
\subsection{Language}
%


==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\textbf{Pose-guided person image synthesis.}
% 这一部分介绍这个任务的方法发展
% Pose-guided person image synthesis任务聚焦于如何在复杂空间中实现pose的转换并尽可能的保留source image的细节特征一致性。这个任务首次由Ma等人提出，早期的工作聚焦于利用conditional 生成对抗网络将source image作为条件信息来引导target图像的生成，如VUNet利用VAE对source image apperance提取并作为条件引入到UNet来生成图片，Def-GAN通过a set of loacl affine transformations和损失约束来对齐不同pose等。这类GAN-based 方法因为模型自身缺乏学习pose空间变换关系的能力导致效果不佳。之后的一些工作有采用flow-based deformation来帮助解构source image的信息以实现pose的对齐，比如GFLA通过计算图片在flow fields的相关性来提取局部注意力特征实现不同区域的对应；也有引入更为详细稠密的补充信息（如UV[Style and Pose Control for Image Synthesis of Humans from a Single Monocular View]，densepose[Controlllable person image synthesis with attribute-decomposed gan]和parsing map来帮助弥补pose之间的inconsistency）。
% 最近的工作采用diffusion作为生成底模，相比于先前gan或其他生成方法在生成高分辨率图像时细节保留差和不稳定的问题，diffusion通过多步forward-backward denoising 过程不仅训练更为稳定，同时也能保留图片的细节特征生成高分辨的图像。PIDM通过设计一个条件texture diffusion模型和disentangle classifier-free guidance机制来实现pose引导下的图像生成，PoCoLD和PCDM分别通过pose constrained attention和progressively 多stage refine来实现pose的对齐。CFLD通过挖掘source image的corse prompt information 然后不断细化来实现细粒度的生成。以上的diffusion-based方法均依赖于预训练的encoder来实现对source image的apeerance信息进行提取，我们认为这类模型因其本身的缺陷（比如数据集的长尾效应）使其关注于常见区域如人脸/手等区域而无法捕捉细粒度的纹理花纹等细节特征，所以导致先前的diffusion-based方法无法生成具有一致性的复杂图案。
PGPIS aims to achieve pose transformation in a complex spatial context while maintaining consistency with the detailed features of the source image, which was initially proposed by Ma \etal ~\cite{ma2017pose}. 
Early approaches~\cite{esser2018variational,ma2017pose} usually employ conditional generative adversarial networks (CGANs) ~\cite{goodfellow2014generative, mirza2014conditional} to guide the generation of target images using the source image as conditional information~\cite{ma2017pose,men2020controllable}. However, due to the significant spatial information differences between the source image and the target image, as well as the sparse guidance from the skeleton map, directly achieving pose transfer is highly challenging. To address the challenges, some works decouple and separately optimize pose and appearance information\cite{ma2018disentangled}, or use attention mechanisms to better establish the mapping relationship between pose and appearance\cite{ren2022neural,zhang2022exploring,zhou2021cocosnet}. 
On the other hands, some approaches introduce more detailed and dense supplementary information, such as UV~\cite{sarkar2021style}, dense-pose~\cite{han2023controllable}, and parsing maps~\cite{men2020controllable,zhang2021pise,zhou2022cross,lv2021learning}, to alleviate inconsistencies between poses. 
Recent approaches adopt diffusion as an alternative generative model\cite{bhunia2023person,shen2024advancing,lu2024coarse,han2023controllable}.By incorporating conditional information into iterative forward-backward denoising procedures~\cite{ho2020denoising}, diffusion-based methods outperform GAN-based approaches in terms of both image generation quality and pose control effectiveness.
PIDM is the pioneering endeavor to integrate the diffusion model into PGPIS, which designs a conditional texture diffusion model and a disentangle classifier-free guidance mechanism~\cite{ho2022classifier}. 
% 加入latent diffusion描述，ldm方法依赖于预训练
PoCoLD and PCDM aim to achieve pose alignment through a pose-constrained attention mechanism and progressive multi-stage refinement, respectively \cite{han2023controllable,shen2024advancing}.
CFLD \cite{lu2024coarse} endeavors to attain coarse-to-fine generation by initially extracting coarse prompt information from the source image, followed by refinement through a learnable Perception-Refined Decoder and Hybrid-Granularity Attention to achieve fine-grained results. 
%

\textbf{Conditional diffusion models.}
% 这一部分介绍条件生成模型的在图片生成发展
The significant potential of diffusion models in traditional unconditional generative tasks has recently been evidenced\cite{ho2020denoising,song2020denoising,song2020score}. 
In contrast to conventional single-step generative models such as Generative Adversarial Networks (GANs)\cite{mirza2014conditional} and Variational Autoencoders (VAEs)\cite{kingma2013auto}, diffusion relies on multi-step denoising sampling of initial noise to generate high-quality data, thereby enabling the production of detailed and diverse outputs. The advancement of various conditional diffusion models further enhances its practicality and versatility. Classifier-free methodologies devise implicit classifiers to guide the weights of controllable and uncontrollable processes, thus facilitating conditional generation\cite{ho2022classifier}. Furthermore, Latent Diffusion Model(LDM)\cite{rombach2022high} utilize denoising process by encoding original images into a low-dimensional latent space and integrate cross-attention mechanisms to introduce multi-modal conditions, thereby significantly expanding the diversity of control information. 
Prior LDM-based approaches\cite{han2023controllable,shen2024advancing,lu2024coarse} rely on pre-trained encoders to extract appearance information from the source image. However, we argue that such encoders have inherent limitations (\ie long tailed biases in dataset), which make them prioritize common regions such as face and hands, and neglect those fine-grained details such as cloth texture patterns.
In contrast, our proposes Siamese conditional diffusion framework excels in capturing complex details and establishing semantic matching, thereby improving the preservation of Full-IDs and ensuring person consistency. Our extensive experimental analysis confirms the limitations of traditional approaches. (\secref{sec:limitation}).
% Recent studies\cite{} have incorporated diffusion models into fashion generation tasks. 
% PCDM introduces a progressive three-stage network consisting of prior-inpainting-refining stages. 
% This model integrates pose alignment relations and utilizes the CLIP model to extract image features, gradually refining image details throughout the three stages. 
% CFLD proposed a coarse-to-fine training paradigm, fully exploiting multiscale information by mining and refining coarse-grained prompts obtained from pre-trained feature extractors (e.g., SwinB) and combining them with a mixed-granularity mechanism. In contrast to previous diffusion-based methods that rely on pre-trained models for extracting semantic or pixel-level appearance details from the source image, this paper introduces a siamese diffusion framework built upon LDM. This framework make full use of the feature extraction and matching abilities of pre-trained diffusion models to blend fine-grained features and facilitate pose transfer within the latent space, achieving higher consistency in pose-guided person image synthesis.

==> sec/3_preliminaries.tex <==
\section{Preliminaries: Diffusion-based PGPIS and Limitations}
\label{sec:preliminary}

% In this section, we briefly introduce the state-of-the-art (SOTA) Diffusion-based PGPIS methods \cite{shen2024advancing,lu2024coarse}. Then, we discuss the limitations of these methods that could be well-addressed by our method introduced in \secref{sec:method}. 

\subsection{Diffusion-based PGPIS }
\label{subsec:diff_pgpis}

Given a source image $\mathbf{I}_\text{s}$, source pose $\mathbf{P}_\text{s}$, and target pose $\mathbf{P}_\tau$, PGPIS aims to generate a target image $\mathbf{I}_\tau$ in which the generated person and their clothes match those in the source image, while the generated person's pose aligns with the target pose.
%
The SOTA diffusion-based PGPIS methods are designed based on the stable diffusion (SD) \cite{rombach2022high} that involves a forward diffusion process and a backward denoising process of $T$ steps.
%
% during the training process, we first use a variational autoencoder (VAE) to extract the latent of ground truth target image $\mathbf{I}_\tau$ (\ie, $\mathbf{z}_\tau$). 
%
The forward diffusion process progressively add random Gaussian noise $\epsilon\in \mathcal{N}(0,\mathbf{I})$ to the initial latent $\mathbf{z}_0$. At the $t$th timestep, we can formulate it as
%
\begin{align} \label{eq:forward_diffusion}
    \mathbf{z}_t = \sqrt{\bar{\alpha}_t}\mathbf{z}_0+ \sqrt{1-\bar{\alpha}_t}\epsilon, t\in[1,T]
\end{align}
%
where $\bar{\alpha}_1,\bar{\alpha}_2,\ldots,\bar{\alpha}_T$ are calculated from a fixed variance schedule. The denoising process uses an UNet to predict the noise, \ie, $\epsilon_\theta(\mathbf{z}_t, t, \mathcal{C},\mathcal{O}_\beta)$ and remove the noise from the latent.
%
The set $\mathcal{C}$ involves related conditions and the function $\mathcal{O}_\beta(\cdot)$ defines the way of embedding condition features into the UNet. 
%
For PGPIS task, we can set  $\mathcal{C} =\{\mathcal{X}_\text{s},\mathcal{X}_\text{tp}, \mathcal{X}_\text{sp}\}$ where $\mathcal{X}_\text{s}$ denotes the features of source image and $\mathcal{X}_\text{tp}$ and $\mathcal{X}_\text{sp}$ contains the features of target pose and source pose.
%
To train the UNet $\epsilon_\theta(\cdot)$, the predicted noise should be the same as the sampled noise during the forward process
%
\begin{align} \label{eq:loss_diffusion}
    \mathcal{L}_\text{mse} = \mathds{E}_{\mathbf{z}_0, \mathcal{C}, \epsilon, t}(\|\epsilon-\epsilon_\theta(\mathbf{z}_t, t, \mathcal{C},\mathcal{O}_\beta)\|^2_2).
\end{align}
%
During the inference with trained $\epsilon_\theta$ and $\mathcal{O}_\beta$, we use image encoder and pose encoder to extract features of the inputs (\ie, $\mathbf{I}_\text{s}$, $\mathbf{P}_\text{s}$, $\mathbf{P}_\text{t}$) and get $\mathcal{C} =\{\mathcal{X}_\text{s},\mathcal{X}_\text{tp},\mathcal{X}_\text{sp}\}$.
%
Then, given the latent $\mathbf{z}_T$, we perform the backward denoising process iteratively to generate the predicted target image. 

\textbf{Coarse-to-fine latent Diffusion (CFLD) \cite{lu2024coarse}.} 
%
The SOTA method CFLD \cite{lu2024coarse} utilizes the pre-trained Swin-B \cite{liu2021swin} to extract multi-layer features (\ie, $\mathcal{X}_\text{s}$) of the source image and the Adapter to extract multi-layer features \cite{mou2023t2i} (\ie, $\mathcal{X}_\text{tp}$) of the target pose. Moreover, CFLD proposes two new modules as the $\text{F}_\beta$ to embed the condition features effectively.

\textbf{Progressive conditional Diffusion models (PCDM) \cite{shen2024advancing}.} Shen \etal proposed three-stage diffusion models to progressively generate high-quality synthesized images. The first stage is to predict the global embedding of the target image; the second stage is to get a coarse target estimation; the final stage is to refine the coarse result. Each stage relies on a diffusion model that could be approximately formulated with \reqref{eq:forward_diffusion} and \reqref{eq:loss_diffusion} with different condition setups. In particular, all three stages use the pre-trained image encoders, \ie, CLIP and DINOv2.

\subsection{Empirical Study}
\label{sec:limitation}

%
\begin{figure}{}{}
% \vspace{-10pt}
    \includegraphics[width=1\linewidth]{figures/fig_anaylsis.pdf}
    % \vspace{-23pt}
    \caption{{Statistical results of attention maps of our method and two SOTA methods.}
    \label{fig:limitation}
    }
% \vspace{-5pt}
\end{figure}
%
As shown in \figref{fig:fig_intro}, the state-of-the-art methods CFLD \cite{lu2024coarse} and PCDM \cite{shen2024advancing} can hardly preserve the clothing patterns and textures.
%
The feature attention maps in \figref{fig:fig_intro} demonstrate a superficial reason, that is, the SOTA methods' features did not focus on the clothing. 
%
To further validate this observation, we perform a statistical analysis.
%
Specifically, we randomly collect 50 examples from the in-shop clothes retrieval benchmark \cite{liuLQWTcvpr16DeepFashion} and use the two SOTA methods to handle these examples.
%
For each sample, we calculate the feature attention map and get its parsing map.
%
Then, we can count the attention values at different parsing regions.
%
After that, we can obtain the average attention values within different regions among all examples.
%
For CFLD, we obtain the feature attention map by calculating the final layer's average value of the softmax layer in the Swin-B. 
%
For PCDM, we follow the steps outlined in the open-source code of PCDM to calculate the attention map.
%
As the results are shown in \figref{fig:limitation}, PCDM using pre-trained CLIP and DINOv2 feature pay less attention to the clothes when we compare the attention values on clothes with the ones on the other two regions.
%
CFLD uses pre-trained Swin-B features, paying less attention to both cloth and head regions.
%
The observation inspires us to design a novel framework, which should encode the source image with both face and cloth key information preserved.
%
Our intuition is to leverage person-parsing maps to guide the image encoding process and inject the parsing-guided embeddings into diffusion generation.

==> sec/4_method.tex <==
\section{Methodology: Person-Parsing-guided Siamese Network Diffusion Model}
\label{sec:method}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/fig_pipeline.pdf}
    \caption{Pipeline of the proposed person-parsing-guided Siamese network diffusion model.}
    \label{fig:pipeline}
\end{figure*}

% In this section, we first introduce the whole framework in \secref{subsec: overview} with the main architecture (\ie, Siamese network diffusion model). Then, we detail the pose-guided parsing projection in \secref{subsec: parsing projection} to estimate the person parsing map of the target image based on the source and target poses and the source image, and the module to extract person-parsing-aligned CLIP embeddings in \secref{subsec: parseclip}. We provide all implementation details in \secref{subsec:implementation}. Please refer to the whole pipeline in \figref{fig:pipeline}.

\subsection{Overview and Siamese Network Diffusion Model}
\label{subsec: overview}

%
Following the task definition of PGPIS, we have inputs including source image $\mathbf{I}_\text{s}$, source pose image $\mathbf{P}_\text{s}$, and target pose image $\mathbf{P}_\tau$.
%
We first employ a person-parsing method \cite{li2020self} to extract the parsing map of $\mathbf{I}_\text{s}$ and get $\mathbf{H}_\text{s}$.
%
Then, we propose to estimate the person-parsing map $\mathbf{H}_\tau$ of the target image by projecting the $\mathbf{H}_\text{s}$ based on the $\mathbf{p}_\tau$ and $\mathbf{p}_\text{s}$, that is,
%
\begin{align}\label{eq:parsing-projection}
    \mathbf{H}_\tau =  \text{ParseProj}(\mathbf{H}_\text{s}, \mathbf{P}_\text{s}, \mathbf{P}_\tau).
\end{align}
%
We will detail the function `\text{ParseProj}' in \secref{subsec: parsing projection} and display an example in the \figref{fig:pipeline}.
%
Then, we employ two encoders (\ie, $\phi_\text{p}$ and $\phi_\text{h}$) to extract embeddings from poses and parsing maps, respectively.
%
Specifically, we have $\mathbf{x}_\text{s} = \phi_\text{p}(\mathbf{P}_\text{s})$, $\mathbf{x}_\tau =\phi_\text{p}(\mathbf{P}_\tau)$, $\mathbf{h}_\text{s} = \phi_\text{h}(\mathbf{H}_\text{s})$, and $\mathbf{h}_\tau =\phi_\text{h}(\mathbf{H}_\tau)$. 
%

Our model is based on the pre-trained stable diffusion (SD) and we can also follow \secref{subsec:diff_pgpis} to generate the target image.
%
The key problem is how to extract the features of the source image effectively, which should turn attention to both face and clothing regions.
%
To this end, we propose to employ pre-trained CLIP and a Siamese network trained by ourselves for image encoding. As discussed in \secref{sec:limitation}, the pre-trained CLIP can capture the human face features well. To preserve this advantage, we propose to extract visual and semantic CLIP embeddings of the target-aligned person region in the source image,
%
\begin{align} \label{eq:pareclip}
    \mathbf{F}_\text{clip} = [\mathbf{F}_\text{clip}^\text{img}, \mathbf{F}_\text{clip}^\text{txt}] =  \text{ParseCLIP}(\mathbf{I}_\text{s},\mathbf{H}_\tau,\mathbf{H}_\text{s}),
\end{align}
%
where $\mathbf{F}_\text{clip}^\text{img}$ and $\mathbf{F}_\text{clip}^\text{txt}$ are CLIP embeddings of the person region and parsing categories, respectively. 
%
We will detail the `\text{ParseCLIP}' in \secref{subsec: parseclip} and present its functionality in the whole pipeline in
\figref{fig:pipeline}.

\textbf{Siamese network diffusion model.} We aim to learn a Siamese network to replace the original UNet for the backward denoising process. 
%
Specifically, the Siamese network contains two UNet branches with the same architectures, which are denoted as SourceNet (\ie, $\epsilon_\theta'(\cdot)$) and TargetNet (\ie, $\epsilon_\theta(\cdot)$). The SourceNet is to extract the multi-level features of the source image and can be formulated as
%
\begin{align} \label{eq:sourcenet}
    \mathcal{F}' = \{\mathbf{F}_l'\}_{l=1}^L = \epsilon_{\theta'}(\mathbf{z}_\text{s},\mathcal{C}', 
    \mathcal{O}_{\beta'}), \text{subject to}~\mathcal{C}'=\{\mathbf{x}_\text{s},\mathbf{h}_\text{s},\mathbf{F}_\text{clip}\}
\end{align}
%
% where $\mathbf{F}_l'$ is the self-attention output of the $l$th layer of $ \epsilon_{\theta'}$. 
where $\mathbf{F}_l'$ is the $l$th-layer attention features of $ \epsilon_{\theta'}$ at $t=0$. 
%
The feature $\mathbf{F}_\text{clip}$ is fused with $\mathcal{F}' = \{\mathbf{F}_l'\}_{l=1}^L$ of $\epsilon_{\theta'}$ via decoupled attention denoted as $\mathcal{O}'_\beta$. 
%
Inspired by \cite{ye2023ip}, we design a new decoupled attention to incorporate image and text simultaneously. 
%
We propose two independent cross-attentions to handle different modalities, and the computation can be formulated as follows:
%
\begin{align} \label{eq:decoupled_attention}
\mathcal{O}'_\beta (\mathbf{F}_\text{clip},\mathbf{F}_l') = g_\text{txt} \cdot \text{Att}(\textbf{Q}_{\mathbf{F}_l'},\textbf{K}_{\mathbf{F}_\text{clip}^\text{txt}},\textbf{V}_{\mathbf{F}_\text{clip}^\text{txt}}) + g_\text{img} \cdot \text{Att}(\textbf{Q}_{\mathbf{F}_l'}, \textbf{K}_{\mathbf{F}_\text{clip}^\text{img}},\textbf{V}_{\mathbf{F}_\text{clip}^\text{img}}),
    % &\text{Att}(\textbf{Q},\textbf{K},\textbf{V})=\text{Softmax}\left(\frac{\textbf{Q} \textbf{K}^{T}}{\sqrt{d}} \textbf{V}\right)
\end{align}
%
where $\text{Att}(\textbf{Q}_*,\textbf{K}_*,\textbf{V}_*)=\text{Softmax}\left(({\textbf{Q}_* \textbf{K}_*^{T}}/{\sqrt{d}})\textbf{V}_*\right)$, and $\{\mathbf{Q}_*,\mathbf{K}_*,\mathbf{V}_* | * \in \{ \mathbf{F}_l', \mathbf{F}_\text{clip}^\text{txt},  \mathbf{F}_\text{clip}^\text{img}\} \}$ are trainable matrices of features in the cross-attention layer. The two variables (\ie, $g_\text{txt}$ and $g_\text{img}$) are weights to combine the two attentions.


The TargetNet (\ie, $\epsilon_\theta$) is to predict noise at the $t$th timestep based on the pose and parsing embeddings, CLIP embeddings, and features extracted from the SourceNet.
%
\begin{align}\label{eq:targetnet}
    \hat{\epsilon} = \epsilon_\theta(\mathbf{z}_t, t, \mathcal{C},\mathcal{O}_\beta), 
    \text{subject to}~\mathcal{C}=\{\mathbf{x}_\tau,\mathbf{h}_\tau,\mathbf{F}_\text{clip},\mathcal{F}'\},
\end{align}
%
where $\mathcal{O}_\beta$ denotes the operations to fuse $\mathcal{F}'$ with the features of $\epsilon_{\theta}$, and the $\mathbf{F}_\text{clip}$ are incorporated in $\epsilon_{\theta}$ via original cross-attentions layer.
%
Specifically, regarding the $lth$ attention feature of $\epsilon_{\theta}$ denoted as $\mathbf{F}_l$, we propose the alignment attention based on \cite{xu2023magicanimate} to fuse $\mathbf{F}_l$ and $\mathbf{F}'_l$, which involves two sub-attentions, \ie, fusion attention and matching attention. The fusion attention facilitates the fusion while matching attention is responsible for extracting and enhancing the features from corresponding regions between $\mathbf{F}_l$ and $\mathbf{F}'_l$. We have the whole formulation as:
%
\begin{align} \label{eq:alignment_attention}
      \mathcal{O}_{\beta}(\mathbf{F}_l, \mathbf{F}'_l) = 
      \text{Att}(\mathbf{W}_q \mathbf{F}_l, \mathbf{W}_k\left[\mathbf{F}_l,\mathbf{F}_l'\right],
      \mathbf{W}_v\left[\mathbf{F}_l,\mathbf{F}_l'\right])+
      %
      \lambda\text{Att}(\mathbf{W}'_{q} \mathbf{F}_l, \mathbf{W}'_{k}\mathbf{F}'_l,\mathbf{W}'_{v} \mathbf{F}'_l), 
\end{align}
%
where $\{\mathbf{W}_*, \mathbf{W}'_* | *\in \{q,k,l\}\}$ are trainable weights, $[ \cdot ]$ concatenates features along the sequence dimension, and $\lambda$ is the control coefficient for corresponding enhancement. The two terms are fusion attention and matching attention, respectively.
For training and inference, we adopt the original SD training objective and sampling strategy, which will be further elaborated in \secref{subsec:implementation}.
% %
% The TargetNet (\ie, $\epsilon_\theta(\cdot)$) is to predict the noise at the $t$th timestep.
% %
% Specifically, we have
% %
% \begin{align} \label{eq:targetnet}
%       \hat{\epsilon} = \epsilon_{\theta} (\mathbf{z}_t,t,\mathcal{C}=\{\mathbf{x}_\text{s},\mathbf{h}_\text{s},\mathbf{F}_\text{clip},\mathcal{F}'\},\mathcal{O}_{\beta}),
% \end{align}
% %
% where 
% %
% where $\mathcal{O}_{\beta}$ contains the alignment attention and cross attention, defining the feature fusion operations.
% %
% We denote the $L$ features of $\epsilon_{\theta}$ as $\mathbf{F}$.
% %
% At the $l$th layer, $\mathbf{F}_\text{clip}$ and $\mathbf{F}_l'\in \mathcal{F}'$ are combined by the alignment attetion while $\mathbf{F}_l$ and $\mathbf{F}_l'$ are fused through the cross attention.


% Then, we can remove the noise at the $t$th timestep via the predicted noise. 
% %
% During the training process, we use the following loss function



\subsection{Pose-guided Parsing Projection}
\label{subsec: parsing projection}

As detailed in \secref{subsec: overview}, the parsing map of the target image is critical for different modules. 
%
However, in the practical, we do not have the target image and cannot use the person-parsing method to predict the parsing map directly.
%
Here, we propose to leverage the source parsing map and the poses of source and target images to estimate the target parsing map (\ie, \reqref{eq:parsing-projection}).
%

To achieve this goal, we follow a similar design to the Siamese network diffusion model. Specifically, we extract the embeddings of the source and target poses via an encoder and get $\mathbf{x}_\tau = \phi_\text{p}(\mathbf{P}_\tau)$ and $\mathbf{x}_\text{s} = \phi_\text{p}(\mathbf{P}_\text{s})$. Then, we calculate the latent of the source parsing map (\ie, $\mathbf{H}_\text{s}$) via VAE and get $\mathbf{z}_\text{hs}$.
%
Similar to \reqref{eq:sourcenet}, we obtain multi-level features of source parsing map through the SourceNet
%
\begin{align} \label{eq:sourcenet_ppp}
    \mathcal{F}' = \{\mathbf{F}'_l\}_{l=1}^L = \epsilon_{\theta'}(\mathbf{z}_\text{hs},\mathcal{C}'), \text{subject to}~\mathcal{C}'=\{\mathbf{x}_\text{s},\mathbf{x}_\tau\},
\end{align}
%
where $\mathbf{F}_l'$ is the $l$th-layer features of $ \epsilon_{\theta'}$ at $t=0$. Then, we use the TargetNet to predict the noise at the $t$th timestep during the backward diffusion process.
%
\begin{align} \label{eq:targetnet_ppp}
      \hat{\epsilon} = \epsilon_{\theta} (\mathbf{z}_t,\mathcal{C},
      \mathcal{O}_\beta), \text{subject to}~\mathcal{C}=\{\mathbf{x}_\text{s},\mathbf{x}_\tau, \mathcal{F}'\}
\end{align}
%
where $\mathbf{F}_l\in \mathcal{F}$ is fused with the $l$th layer of $\epsilon_{\theta}$ through the aligntment attention.
%
Then, we remove the noise at the $t$th timestep via the predicted noise. 
%
Note that, we use the same architectures for the pose encoder, SourceNet, and TargetNet as the ones in \secref{subsec: overview}. However, their weights are not shared.


\subsection{Person-Parsing-aligned CLIP Embedding Extraction}
\label{subsec: parseclip}

As introduced in \secref{subsec: overview}, we aim to extract CLIP embeddings of the target-aligned person region in the source image.
%
Given the source parsing map $\mathbf{H}_\text{s}$ and target parsing map $\mathbf{H}_\tau$, we first perform category matching. 
%
We have the category sets $\mathcal{V}_\text{s}$ and $\mathcal{V}_\tau$ of the source and target parsing maps, which involves the categories included in the two maps.
%
For example, we could have $\mathcal{V}_\text{s}=\{\text{`head',`face',`shirt',`pant',\ldots}\}$ and
%
each category in the set corresponds to a region in the parsing map.
%
Then, we remove the categories that are within $\mathcal{V}_\text{s}$ but not within $\mathcal{V}_\text{t}$ from $\mathcal{V}_\text{s}$ and get $\hat{\mathcal{V}}_\text{s}$.
%
As a result, the category-related regions in the parsing map $\mathbf{H}_\text{s}$ are set as zero and we obtain a new source parsing map denoted as $\hat{\mathbf{H}}_\text{s}$.
%
After that, we can get a tight bounding box tightly wrapped in the person region in $\hat{\mathbf{H}}_\text{s}$.
%
We use this bounding box to crop the source image and get $\hat{\mathbf{I}}_\text{s}$. 
%
We leverage the CLIP visual and text encoders to extract the embeddings of $\hat{\mathbf{I}}_\text{s}$ and $\hat{\mathcal{V}}_\text{s}$, respectively.

\subsection{Implementation Details}
\label{subsec:implementation}

\textbf{Optimization and sampling.}
%
During the training process, we also adopt classifier-free guidance \cite{ho2022classifier}, which is a strategy widely used in diffusion models to enhance the quality and control of the generated images. To achieve that we set conditions $\mathcal{C}$ to 0 with a random probability of $\eta$\%.
The final training loss function is rewritten as
%
\begin{align} 
    \label{eq:saimese_loss}
      \mathcal{L} = \mathds{E}_{\mathbf{z}_0, \mathcal{C}, \epsilon, t}(\|\epsilon-\epsilon_\theta(\mathbf{z}_t, t, \mathcal{C},\mathcal{O}_\beta)\|^2_2).
\end{align}
%
For ParseProj training, we estimate the parsing map and skeleton map of DeepFashion dataset using \cite{li2020self} and \cite{yang2023effective}, respectively. It is worth noting that during the training process of ParseProj, only the Alignment attention and PoseEncoder are trained.
For Saimese network, we employ the projected $\mathbf{H}_\tau$ and other estimated mapping results for training. All modules in Saimese network are involved in the training process except for VAE and CLIP remain fixed. 
%

In inference phase, given a randomly initialized Gaussian noise, we utilize the TargetNet (\ie, $\epsilon_\theta(\cdot)$) to predict the noise at the $t$th timestep and employ classifier scale $\omega$ to regulate the strength of guidance. The sampling formula is as follows:
\begin{align} 
    \label{eq:inference}
    \hat{\epsilon}_{t}=\epsilon_{\theta}(z_t,t,\varnothing,\varnothing) + \omega \cdot(\epsilon_{\theta} (\mathbf{z}_t,t,\mathcal{C},\mathcal{O}_{\beta})-\epsilon_{\theta}(z_t,t,\varnothing,\varnothing)).
\end{align}
Target latents can be obtained through multi-step denoising process, and mapping them back to the original image space we can acquire the target images. 


\textbf{Model details.}
Our Siamese network is derived by modifying the structure and weights of Stable Diffusion v2.1, based on the Hugging Face Diffusion library. Both PoseEncoder and ParseEncoder are a lightweight network with four convolutional layers. 
For training, we run on 4 NVIDIA A800 GPUs, with a batch size of 12 for $512\times 352$ and batch size of 60 for $256\times 176$. The training process consists of 100 epochs and uses the AdamW optimizer with a fixed learning rate of $1e^{-5}$. Classifer-free dropout probability $\eta$ is 30\%. For inference, We employ the DDIM\cite{ho2020denoising} scheduler with a sampling step of 35 and set classifier scale $\omega$ to 2.5. More details are explained in \secref{subsec:appendix_detail}.
%


==> sec/5_experiments.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figures/fig_qualitative_comparison.pdf}
    \caption{Qualitative comparisons \protect\\with SPGNet \cite{lv2021learning}, CASD \cite{zhou2022cross}, DPTN \cite{zhang2022exploring}, PIDM \cite{bhunia2023person}, NTED \cite{ren2022neural}, PCDM \cite{shen2024advancing} and CFLD \cite{lu2024coarse}.}
    \label{qualitative_figure}
    % \vspace{-10pt}
\end{figure*}
%
\section{Experiments}
\subsection{Setup}
\textbf{Dataset.}
% 这一段主要介绍数据集的构建
We follow \cite{shen2024advancing,lu2024coarse} to conduct extensive experiments on In-Shop Clothes Retrieval benchmark from DeepFashion dataset and evaluated on 512$\times$352 and 256$\times$176 resolutions respectively. 
The dataset is comprised of 52,712 high-resolution images featuring clean backgrounds and diverse fashion models. 
To be consistent with the configuration in PATN~\cite{zhu2019progressive}, we split this dataset into non-overlapping training and testing set with 101,966 and 8,570 pairs, respectively, with each pair including a source image and its corresponding target image.

% It is noteworthy that the person identities in both the training and testing sets for both datasets do not overlap.
% \par
\textbf{Objective metrics.}
% 这一段介绍客观的指标，比如ssim psnr fid
We use four widely used metrics, namely \textit{Structure Similarity Index Measure} (SSIM) \cite{wang2004image}, \textit{Peak Signal to Noise Ratio} (PSNR), \textit{Learned Perceptual Image Patch Similarity} (LPIPS) \cite{zhang2018unreasonable}, and \textit{Fr$\acute{e}$chet Inception Distance} (FID) \cite{heusel2017gans}, to assess quality and fidelity of generated images. 
% The four metrics differ in the way they measure the similarity (distance) between two images or datasets.
% LPIPS uses a model trained on human judgments to measure perceptual similarity, while SSIM considers aspects such as brightness, contrast, and structure. 
% PSNR quantifies the degree of distortion. FID calculates the Wasserstein-2 distance~\cite{vaserstein1969markov} on the distribution of the two data sets.
% \par

\textbf{Subjective metrics.}
% 主观指标，调研问卷等
% Considering that objective metrics cannot fully capture human perception of how similar two images are, which is usually subjective,
We employ three subjective metrics as referenced in the literature \cite{bhunia2023person}: R2G \cite{ma2017pose}, G2R \cite{ma2017pose}, and J2b \cite{siarohin2018deformable,bhunia2023person}.
%
R2G and G2R represent the ratios of real images classified as generated images and generated images classified as real images, respectively. Higher values for R2G and G2R indicate a greater similarity to real images. Meanwhile, J2b reflects user preferences by comparing the proportion of users selecting the best image from a group of images generated by different methods.



\subsection{Quantitative and qualitative comparison}
\label{subsec:quantitative and qualitative comparison}
%
\begin{table*}[t!]
    \centering
    % \renewcommand\arraystretch{1}
    % \setlength{\tabcolsep}{20pt}
    \caption{Quantitative comparisons with the state of the arts in terms of image quality. $^\dagger$We reproduce these results based on the checkpoints instead of generated images provided by the authors. $^\ast$Results are cited from PoCoLD without publicly available checkpoints or generated images. Others are cited from NTED.}
    \label{tab:main_experiment}
    \resizebox{1\linewidth}{!}{
    \input{tab/tab_quantitative}
    }
\end{table*}
%
% \todo{First briefly summarize what this subsection serves for.}
We conducted a comprehensive comparison with SOTA approaches including GAN-based, flow-based, attention-based and diffusion-based ones, they are PATN~\cite{zhu2019progressive}, ADGAN~\cite{men2020controllable}, GFLA~\cite{ren2020deep}, 
SPGNet\cite{lv2021learning},
PISE~\cite{zhang2021pise}, CASD~\cite{zhou2022cross}, CocosNet2~\cite{zhou2021cocosnet}, NTED~\cite{ren2022neural}, DPTN~\cite{zhang2022exploring}, PIDM~\cite{bhunia2023person}, PoCoLD~\cite{han2023controllable}, PCDM~\cite{shen2024advancing}, and CFLD~\cite{lu2024coarse}. 
Additionally, we perform a qualitative evaluation of the latest seven SOTA methods.
% among which PIDM, CFLD, and PCDM are diffusion-based approaches.

\textbf{Quantitative comparison.}
% 主要是表格的分析
% 我们与11种SOTA方法在四个指标上进行了quantitative comparison，结果如表1所示。在第一组分辨率对比中，我们在3/4的指标中超过其他方法，其中远超flow-based和gan-based的方法。值得注意的是我们在由human judgements上训练得到的指标LPIPS中远超其他方法，表示我们的方法在图像的重建上更符合人类审美。尽管我们在FID指标上略高于PIDM，但这可能是PIDM过度拟合了数据集的分布所导致。此外先前的工作也表明FID并不能完全代表图像生成的好坏。我们在第二组实验中相比于其他方法取得了更大的优势，远超其他三类LDM-based的方法。值得注意的是，由于PoCoLD没有提供任何公开的结果导致无法对其进行相同环境下的定量评价，故不纳入最终比较
We perform a quantitative comparison with 11 SOTA methods across four metrics (See \tableref{tab:main_experiment}). In 256$\times$176 resolution comparison, our method outperforms others in 3 out of 4 metrics, particularly showing a substantial lead over flow-based and GAN-based methods. Notably, in the metric LPIPS, which is trained using human judgments, our method significantly outperforms other approaches. This indicates that our method better aligns with human aesthetics in terms of image reconstruction. While our FID metric slightly exceeds that of PIDM, this can potentially be attributed to PIDM overfitting the dataset distribution as also discussed in prior research\cite{shen2024advancing,lu2024coarse,han2023controllable}, and they has also suggested that FID does not fully reflect the quality of image generation.
%
\begin{figure}{}{}
% \vspace{-12pt}
    \includegraphics[width=\linewidth]{figures/fig_user_study.pdf}
    % \vspace{-23pt}
    \caption{{\color{black}User study results in terms of R2G,G2R and Jab metrics. Higher values in metrics means better quality of generated results.}
    \label{user study}
    }
% \vspace{-12pt}
    \label{fig:problem}
\end{figure}
%
In the second set of experiments, our method demonstrates a significant advantage over other approaches, surpassing all three categories of LDM-based methods. It is worth noting that PoCoLD\cite{han2023controllable} does not provide any publicly available results, which hinders us from conducting a quantitative evaluation under the same conditions.
Therefore, it is excluded from the final comparison. 
% Additionally, we also provide the metrics results of VAE reconstructed and ground truth as references for comparison.

\textbf{Qualitative comparison.}
% 主要是图片主观层面的分析
In \figref{qualitative_figure}, we present the results where our framework is compared to the various types of SOTA methods in DeepFashion dataset and the four objective metrics. 
% From left to right, it consists of source images, target poses, generated images of different approaches in comparison, and target images ('Ground Truth').
%
We observer that: 
\ding{182} When confronted with extreme pose variations or extensive occlusions as demonstrated in the images in \textit{rows 1-3}, only diffusion-based methods (\textit{columns 7-10}) are capable of reconstructing the approximate pattern outlines of the clothing and faces, and our method significantly outperforms others in terms of face and cloth ID preservation and consistency. This superiority stems from our ability to explore deeper spatial and semantic matching information, followed by enhanced feature fusion achieved through Siamese networks. 
\ding{183} Addressing the challenge of reconstructing intricate patterns such as designs and text, which previous methods struggle with (as observed in all rows), our approach leverages the Siamese diffusion framework to better retain fine-grained details under significant scale variations. Compared to others, our method preserves finer details, resulting in less disparity from real images.
\ding{184} The last two rows indicate that irrespective of minor or giant pose differences, our method maximizes the retention of structural clothing features from the source image. As evidenced in the fifth line, only our approach accurately preserves features such as suspender designs.
More examples and ParseProj qualitative results are listed in \secref{subsec:appendix_qualitative_compare}.

\textbf{User study.}
% 以上定量和定性的结果比较展示了我们相较于其他方法的显著优势，然而定量的结果仍然不能完全反映图像细节上的差异（比如花纹，文字等）。为了更好的反映我们方法在细节一致性保持的优势，我们完全参照PIDM的实验设置对30名有着计算机背景的志愿者开展了一项用户研究。(1)针对R2G和G2R两项指标，我们从每种生成方法和真实数据集中各随机挑选30张图片组成一组测试数据，志愿者需要判别每张图片是否为生成图片。可以看出我们在G2R上显著优于其他方法，有一半以上的图片被认为是真实的，这反映了我们生成的图片难以被辨别，更趋近真实图片。此外相比之下R2G指标在各类方法中没有显著差异。(2)针对jab指标，为了更好的凸显我们方法的优越性，我们分别进行了两组实验，一组为挑选后的30张具有复杂花纹和文字的图片，另一组为随机挑选的30张图片来进行公平的对比。可以发现两组数据集上我们均显著优于其他方法(70.2和53.6)，表明我们的方法在复杂图像一致性保持上远超其他方法。
% 用户主观分析,这里需要放一个类似这种表的对比图，包含了三个指标
% The quantitative and qualitative comparisons presented above demonstrate the significant advantages of our approach over others.
% However, quantitative results still fail to fully exhibit the differences in image details (such as textures, text, etc.). 
%
To better illustrate the advantage of our method, we further conduct a user study involving 30 volunteers with a background in computer science, following the experimental setup of PIDM \cite{bhunia2023person} completely.
%
As shown in \figref{user study}, we can make the following observations:
\ding{182} For the R2G and G2R metrics, we randomly select 30 images from each generation method and the real dataset to form a test dataset. Volunteers were required to discern whether each image was generated or real. Our method significantly outperforms other methods in terms of the G2R metric, with over half of the images being perceived as real. Furthermore, there were no significant differences in the R2G metric among the various methods.
\ding{183}  We also conduct two Jab experiments. In one set, we select 30 images with complex patterns and text generated by each method. In the other set, we randomly select 30 images generated by each method for fair comparison. Our method significantly outperformed others on both sets of datasets, achieving scores of 70.2 and 53.6 respectively. These results clearly indicate that our approach surpasses other methods by a wide margin in terms of preserving consistency in both complex and normal images, while also exhibiting a stronger alignment with human aesthetics. More detailed information are explained in \secref{subsec:user_study}.

\textbf{Ablation study.}
%
\begin{table}
    \centering
    % \renewcommand\arraystretch{1}
    % \setlength{\tabcolsep}{20pt}
    \caption{Ablation study on different contributions.}
    \label{tab:ablation}
    \resizebox{1\linewidth}{!}{
    \input{tab/tab_ablation}
    }
\end{table}
%
To demonstrate the effectiveness of our contributions, we conduct ablation experiments on DeepFashion as shown in \tableref{tab:ablation_3}. 
% 
\textbf{B1} represents our adoption of pre-trained encoders (\ie CLIP) to extract information from the source images, and then we introduce the extracted information into TargetNet via vanilla cross-attentions. 
%
\textbf{B2} is a variant without Siamese network. We design a stacked multi-layer perceptron (MLP) to map the extracted features from CLIP to the shape of the $lth$ layer in TargetNet, enabling feature incorporation within the same fusion setup.
%
In both B1 and B2, regardless of the fusion approach, it has been demonstrated that CLIP encoders cannot fully extract detailed information, resulting in poor performance across all three metrics. 
%
To better capture fine-grained information, we introduced the Siamese network into \textbf{B4} and \textbf{B3}. All three metrics showed significant improvements, particularly LPIPS and SSIM, which are indicators reflecting image authenticity and human preferences. 
% It is worth noting that there is still a certain gap compared to the SOTA methods. 
We further proposed ParseProj and ParseCLIP to provide semantic-level matching information and region enhancement. Here, B4 represents the absence of ParseProj, and B3 represents the absence of ParseCLIP. The results demonstrate the effectiveness of both modules. Qualitative results of the ablation study can be confirmed in \secref{subsec:appendix_ablation}.


==> tab/tab_application.tex <==

\begin{tabular}{l|c|c|c}
    \toprule[0.3pt]
    % \multirow{14}{*}{\makecell{DeepFashion \\ (256$\times$176)}} 
    \multicolumn{3}{c|}{\textbf{Percentage of real images}} &
        \multirow{2}{*}{\textbf{Method}} &   
        % \cmidrule(lr){2-4}\cmidrule(lr){5-7}
        & \textbf{20\%}   & \textbf{60\%}   & \textbf{100\%}          \\
        \midrule 
    \midrule[0.2pt]
    Standard        &  &  &  \\
    \midrule[0.2pt]
    PCDM           &  &  &   \\
    CFLD             &  &  &   \\
    \textbf{Ours}           &  &  &  \\
    \bottomrule[0.3pt]
\end{tabular}


==> tab/tab_quantitative.tex <==

\begin{tabular}{c l c c c c c c c}
    \toprule
        \textbf{Dataset} & \textbf{Method} & \textbf{Venue} & \textbf{LPIPS$\downarrow$} & \textbf{SSIM$\uparrow$} & \textbf{PSNR$\uparrow$} & \textbf{FID$\downarrow$} & \textbf{IQA(Aesthetic)$\uparrow$} & \textbf{IQA(Quality)$\uparrow$}  \\
    \midrule
        \multirow{14}{*}{\makecell{DeepFashion \\ (256$\times$176)}} 
             &  PATN\cite{zhu2019progressive} & CVPR 19' & 0.2533 & 0.6714 & - & 20.728 & - & -\\
             &  ADGAN$^\dagger$\cite{men2020controllable} & CVPR 20' & 0.2255 & 0.6735& 17.010 & 14.540 & 0.2504 & 0.5825\\
             &  GFLA\cite{ren2020deep} & CVPR 20' & 0.1878 & 0.7082& - & 9.827 & - & - \\
             &  PISE$^\dagger$\cite{zhang2021pise} & CVPR 21' & 0.2244 & 0.6537& 13.645 & 11.518 & 0.2185 & 0.5354\\
             &  SPGNet$^\dagger$\cite{lv2021learning} & CVPR 21' & 0.2345 & 0.6913& 17.198 & 16.254  & 0.2756 & 0.5540\\
             &  CASD$^\dagger$\cite{zhou2022cross} & ECCV 22' & 0.1956 & 0.7201 & 17.562 & 13.064 & 0.2532 & 0.5980 \\
             &  NTED$^\dagger$\cite{ren2022neural} & CVPR 22' & 0.1752 & 0.7182 & 17.540 & 8.684 & 0.3088 & 0.5978\\
             &  DPTN$^\dagger$\cite{zhang2022exploring} & CVPR 22' & 0.2004 & 0.7107 & 17.032 & 17.526 & 0.1582 & 0.3797 \\
             &  PIDM$^\dagger$ \cite{bhunia2023person} & CVPR 23' & 0.1867 & 0.6765 & 16.185 & \textbf{6.663} & \underline{0.3284} & 0.5697 \\
             &  \color{gray}PoCoLD$^\ast$\cite{han2023controllable} & \color{gray}ICCV 23' & \color{gray}0.1642 & \color{gray}0.7310 & - & \color{gray}8.067 & - & - \\
             &  PCDM$^\dagger$\cite{shen2024advancing} & ICLR 24' & \underline{0.1633} & \underline{0.7250} & 17.828 & 7.741 & 0.2972 & 0.6926\\   %生成图
             &  CFLD$^\dagger$\cite{lu2024coarse} & CVPR 24' & 0.1768 & 0.7225 & \underline{17.883} & 7.326 & 0.3253 & \underline{0.6931} \\    %生成图
             &  \textbf{Ours} &  & \textbf{0.1509} & \textbf{0.7272} & \textbf{18.123} & \underline{7.265} & \textbf{0.3448} & \textbf{0.7249}\\
    \midrule
        \multirow{7}{*}{\makecell{DeepFashion \\ (512$\times$352)}} 
            & CocosNet2\cite{zhou2021cocosnet} & CVPR 21' & 0.2265 & 0.7236 & - & 13.325 & - & -\\
             & NTED$^\dagger$\cite{ren2022neural} & CVPR 22' & 0.1998 & 0.7356 & 16.3918 & 7.633 & 0.5470 & 0.8282 \\
             & \color{gray}PoCoLD$^\ast$ \cite{han2023controllable} &  \color{gray}ICCV 23' &  \color{gray}0.1920 &  \color{gray}0.7430 & - &  \color{gray}8.416 & - & -\\
             & PCDM$^\dagger$\cite{shen2024advancing} & ICLR 24' & \underline{0.1984} & 0.7273 & 17.013 & 7.147 & 0.5105 & 0.8665 \\ %生成的图
             & CFLD$^\dagger$\cite{lu2024coarse} & CVPR 24' & 0.2018 & \underline{0.7343} & \underline{17.101} & \underline{7.102} & \underline{0.5548} & \underline{0.8842} \\ %生成的图
             & \textbf{Ours} &  & \textbf{0.1803} & \textbf{0.7444} & \textbf{17.627} & \textbf{7.055} & \textbf{0.5666} & \textbf{0.8953} \\
             &  \color{gray} Ground Truth &  & \color{gray}0.0000 & \color{gray} 1.0000 & \color{gray} $+\infty$  & \color{gray} 8.028 & \color{gray} 0.5715 & \color{gray} 0.9478\\
    \midrule
        \multirow{4}{*}{\makecell{WPose \\ (512$\times$352)}} 
            & PCDM$^\dagger$\cite{shen2024advancing} & ICLR 24' & \underline{0.6828} & 0.2611 & \underline{10.429} & - & 0.3264 & 0.1986  \\
            & CFLD$^\dagger$\cite{lu2024coarse} & CVPR 24' & 0.7089 & \underline{0.3269} & 9.789 & - & \underline{0.4706} & \underline{0.2713}  \\
            & \textbf{Ours} & & \textbf{0.5835} & \textbf{0.3311} & \textbf{11.457} & - & \textbf{0.5656} & \textbf{0.3371} \\
            &  \color{gray} Ground Truth &  & \color{gray}0.0000 & \color{gray} 1.0000 & \color{gray} $+\infty$ & - & \color{gray} 0.8390 & \color{gray} 0.5284 \\
    \toprule
\end{tabular}
    % Dataset & \makecell{Method} & Venue & LPIPS$\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & FID$\downarrow$\\
    % IQA(Aesthetic)$\uparrow$ & IQA(Quality)$\uparrow$
    % \midrule
    %     \multirow{14}{*}{\makecell{DeepFashion \\ (256$\times$176)}} 
    %      &  PATN\cite{zhu2019progressive} & CVPR 19' & 0.2533 & 0.6714 & - & 20.728 & - & -\\
    %      &  ADGAN\cite{men2020controllable} & CVPR 20' & 0.2255 & 0.6735& - & 14.540 & 0.2504 & 0.5825\\
    %      &  GFLA\cite{ren2020deep} & CVPR 20' & 0.1878 & 0.7082& - & 9.827 & - & - \\
    %      &  PISE\cite{zhang2021pise} & CVPR 21' & 0.2244 & 0.6537& - & 11.518 & 0.2185 & 0.5354\\
    %      &  SPGNet^\dagger$\cite{lv2021learning} & CVPR 21' & 0.2345 & 0.6913& 17.198 & 16.254  & 0.2756 & 0.5540\\
    %      &  CASD$^\dagger$\cite{zhou2022cross} & ECCV 22' & 0.1956 & 0.7201 & 17.562 & 13.064 & 0.2532 & 0.5980 \\
    %      &  NTED\cite{ren2022neural} & CVPR 22' & 0.1752 & 0.7182 & - & 8.684 & & 0.3088 & 0.5978\\
    %      &  DPTN$^\dagger$\cite{zhang2022exploring} & CVPR 22' & 0.2004 & 0.7107 & 17.032 & 17.526 & 0.1582 & 0.3797 \\
    %      &  PIDM$^\dagger$ \cite{bhunia2023person} & CVPR 23' & 0.1867 & 0.6765 & 16.185 & \textbf{6.663} & 0.3284 & 0.5697 \\
    %      &  \color{gray}PoCoLD$^\ast$\cite{han2023controllable} & \color{gray}ICCV 23' & \color{gray}0.1642 & \color{gray}0.7310 & - & \color{gray}8.067 & - & - \\
    %      &  PCDM$^\dagger$\cite{shen2024advancing} & ICLR 24' & \underline{0.1633} & \underline{0.7250} & 17.828 & 7.741 & 0.2972 & 0.6926\\   %生成图
    %      &  CFLD$^\dagger$\cite{lu2024coarse} & CVPR 24' & 0.1768 & 0.7225 & \underline{17.883} & 7.326 & \underline{0.3253} & \underline{0.6931} \\    %生成图
    %      &  \textbf{Ours} &  & \textbf{0.1509} & \textbf{0.7272} & \textbf{18.123} & \underline{7.265} & \textbf{0.3448} & \textbf{0.7249}\\
    %      % &  \color{gray} VAE Reconstructed & & \color{gray}0.0104 & \color{gray}0.9660 & \color{gray} 33.515 & \color{gray} 8.235  \\
    %      &  \color{gray} Ground Truth &  & \color{gray}0.0000 & \color{gray} 1.0000 & \color{gray} $+\infty$ & \color{gray} 7.952 \\
    % \midrule 
    %      \multirow{8}{*}{\makecell{DeepFashion \\ (512$\times$352)}} 
    %      & CocosNet2\cite{zhou2021cocosnet} & CVPR 21' & 0.2265 & 0.7236 & - & 13.325 \\
    %      & NTED\cite{ren2022neural} & CVPR 22' & 0.1980 & 0.7376 & - & 7.782 \\
    %      &  \color{gray}PoCoLD$^\ast$ \cite{han2023controllable} &  \color{gray}ICCV 23' &  \color{gray}0.1920 &  \color{gray}0.7430 & - &  \color{gray}8.416 \\
    %      % & PCDM$^\ddagger$ & ICLR 24' & 0.1731 & 0.7471 & 18.028 & 7.499 \\ %提供的图
    %      & PCDM$^\dagger$\cite{shen2024advancing} & ICLR 24' & \underline{0.1871} & 0.7311 & \underline{17.282} & 7.542 \\ %生成的图
    %      % & CFLD$^\dagger$ & CVPR 24' & 0.1818 & 0.7478 & 17.652 & 0.896 \\ 提供的图
    %      & CFLD$^\dagger$\cite{lu2024coarse} & CVPR 24' & 0.1993 & \underline{0.7394} & 17.088 & \underline{7.394} \\ %生成的图
    %      & \textbf{Ours} &  & \textbf{0.1728} & \textbf{0.7493} & \textbf{17.699} & \textbf{6.577} \\
    %      % &  \color{gray} VAE Reconstructed &  & \color{gray} 0.0294 & \color{gray} 0.9278 &\color{gray}31.312 & \color{gray} 8.260 \\
    %      &  \color{gray} Ground Truth &  & \color{gray}0.0000 & \color{gray} 1.0000 & \color{gray}  & \color{gray} 8.028 \\
    % \toprule


